Neural Recursive Belief States in Multi-Agent Reinforcement Learning

In multi-agent reinforcement learning, the problem of learning to act is particularly difficult because the policies of co-players may be heavily conditioned on information only observed by them. On the other hand, humans readily form beliefs about the knowledge possessed by their peers and leverage beliefs to inform decision-making. Such abilities underlie individual success in a wide range of Markov games, from bluffing in Poker to conditional cooperation in the Prisoner's Dilemma, to convention-building in Bridge. Classical methods are usually not applicable to complex domains due to the intractable nature of hierarchical beliefs (i.e. beliefs of other agents' beliefs). We propose a scalable method to approximate these belief structures using recursive deep generative models, and to use the belief models to obtain representations useful to acting in complex tasks. Our agents trained with belief models outperform model-free baselines with equivalent representational capacity using common training paradigms. We also show that higher-order belief models outperform agents with lower-order models.

==> Neural Recursive Belief States in Multi-Agent Reinforcement Learning Arxiv_v2/main.tex <==
\section{Introduction}

Partially observable Markov games \cite{Littman:1994:MGF:3091574.3091594, Hansen:2004:DPP:1597148.1597262} (POMGs) are the most general and most challenging category of learning problems for multi-agent systems. Here, agents may have competing goals, the full state of the world is not observable, and the environment appears non-stationary to any individual, by virtue of the learning dynamics of their co-players.\footnote{In a sense, multi-agent problems are generically partially observable, since the policy distributions of each player are not usually common knowledge at each point in time, whereas sampled actions may be observed.}  Multi-agent reinforcement learning (MARL) \cite{4445757} provides a method for learning capable policies in POMGs. However, the equilibria found by model-free systems are not necessarily optimal from the perspective of the individual or the collective. Different types of POMGs present unique failure modes. In competitive settings, agents may learn to play an unexploitable strategy, rather than adapting to the weaknesses of their opponents for greater payoff, as discussed in \cite{vezhnevets2019options}. If the environment is a social dilemma, MARL often converges to defecting equilibria, motivated by greed or fear, see for example \cite{DBLP:journals/corr/abs-1803-08884, DBLP:journals/corr/LererP17}. Coordination problems typically have multiple equilibria, and selecting the best is an extremely hard joint exploration problem; see \cite{Claus:1998:DRL:295240.295800} for instance. To address these difficulties, we can leverage a belief model over the unobserved parts of the world, comprising the private information of other players and their policies. This is often referred to as opponent modelling \cite{DBLP:journals/ai/AlbrechtS18}, although it may be applied outside of purely competitive situations. In the human behavioral literature, this ability is known as theory of mind \cite{premack_woodruff_1978, doi:10.1080/17405629.2018.1435413}. Prior work has shown success in the tabular setting by learning belief models with frequentist \cite{Chang2001PlayingIB, Makino:2006:MRL:1160633.1160772} and Bayesian \cite{Chalkiadakis:2003:CMR:860575.860689} statistical estimation. However, scaling these approaches beyond small tabular settings is notoriously difficult \cite{doshi}.

With the advent of deep reinforcement learning (RL), it has become tractable to learn embeddings which represent the policies of others \cite{rabinowitz2018machine}. However, combining such learning with an adaptive rule which simultaneously leverages the model remains a difficult challenge. In many settings, fortunately, we have access to interpretable representations of the world that are valuable for the task at hand; an example of such is the private information of others. Indeed, the mental states that humans attribute to others are often characterized as representing private information about the world \cite{byom}. We leverage a learned predictive model of such representations as input to the policy. Crucially, we do not otherwise alter the policy update, allowing us to retain the scalability and domain-agnosticism of deep RL. Furthermore, our method includes the recursive reasoning \cite{stahl1995players} characteristic of humans, by learning models over the belief states of other players. 

The method we propose learns beliefs using recursive deep generative models, which are designed to provide useful representations for acting in multi-agent tasks.
In our experiments, we demonstrate that agents equipped with these belief models learn to leverage the behavior of their co-players to maximize rewards in an intricate partially observable gridworld domain (Running with Scissors \cite{vezhnevets2019options}).


\section{Methods}
\subsection{Partially observable Markov games}
\label{sec:belief_models}

Partially Observable Markov Decision Processes (POMDPs) provide a general framework to study the behavior of a solitary, rational agent interacting with an environment whose true state $S_t$ is unknown to the agent. At every time-step, the agent receives sensory observation $Y_t$, sampled from the observation distribution $p(Y_t|S_t)$. The agent uses all the information known, the \textit{history} of all past observations $H_t = (Y_{\leq t}, A_{\leq t-1})$, to take an action $A_t$ sampled from the policy $\pi(A_t|H_t)$. The agent receives a reward $R_t(S_t,A_t)$ and the environment state changes according to its transition dynamics $p(S_{t+1}|S_t,A_t)$. The aim of the agent is to maximize the expected sum of discounted rewards. A particular challenge in POMDPs is the growth of relevant information available to the agent over time: it is not clear how to maintain a concise representation of knowledge which is sufficient to compute optimal decisions. Given an appropriate prior, the observation distribution and transition dynamics, one can compute by Bayes' rule the posterior distribution $p(S_t|H_t)$ over the true state of the environment given all information available at time $t$. A key result \cite{astrom1965optimal} states that this is sufficient to compute an optimal policy; this quantity is called the \emph{belief state} (or belief for short) and represents the knowledge an agent has over the true state of the world. Classically, belief states were represented by simple distributions and computed by explicit Bayesian filtering \cite{ross2011bayesian}, which limited their applicability to complex environments. However, a recent body of work
has been leveraging deep learning techniques to represent a belief state by a neural code $\hat{b}_t$. This code is computed by a recurrent neural network (RNN) $\hat{b}_t\defeq\text{RNN}(\hat{b}_{t-1}, Y_t)$, and follows an update mimicking the Bayesian filter. This code can be decoded to a state distribution by a deep generative model $p(S_t|\hat{b}_t)$. These \emph{neural belief states} are either learned using supervision on state information \cite{moreno2018neural,humplik2019meta}, or learned indirectly through unsupervised learning \cite{venkatraman2017predictive,IglZLWW18,GregorPBBW19,guo2018neural,zhang2019learning,gregor2019shaping}.

Single-agent POMDPs can be extended to the multi-agent setting by considering \emph{partially observable Markov games} (POMG)~\cite{Littman:1994:MGF:3091574.3091594, Hansen:2004:DPP:1597148.1597262}, a general and challenging category of learning problems for multi-agent systems. Very closely related notions can be found in the literature, for instance iPOMDPs \cite{gmytrasiewicz2005framework, han2018learning, doshi2009monte, han2019ipomdp}, and imperfect information games in game theory, see e.g.~\cite{brown2018depth}. In this setting, agents may have competing goals, the full state of the world is not observable, and the environment appears non-stationary to any individual, by virtue of the learning dynamics of their co-players. At each time-step $t$, players $i=1,\dots,n$ share the environment state $S_t$. They each receive an observation $Y_t(i)$ drawn from $p(Y_t(i)|S_t, i)$ and form a history $H_t(i) = (Y_{\leq t}(i), A_{\leq t-1}(i))$ used to compute an action $A_t(i)$ from their own policy $\pi_i(A_t(i)|H_t(i))$. They receive a reward $R_t(S_t, \mathbf{A}_t)$, where $\mathbf{A}_t$ denotes the joint action $(A_t(1),\ldots, A_t(n))$, and the common state changes according to $p(S_{t+1}|S_t, \mathbf{A}_t)$. 

Following the reasoning from POMDPs, it intuitively makes sense for each agent to compute a belief state representing their own uncertainty about the state of the environment. For reasons which will become clear shortly, we call such a belief state a \textit{zeroth-order belief}, and denote it $B^0_t(i)$ for agent $i$. From the perspective of a single agent, when the policies of other agents are fixed, the POMG appears as a POMDP: the other agents become part of the environment, and the unknown state of the world is therefore not only the environment state $S_t$, but also the state of knowledge of other agents. For that reason, agent $i$ has to form a belief about other agents' beliefs, which are \emph{first-order beliefs}. This leads to a recursion, where agents can now form \emph{second-order beliefs} about other agents' first-order beliefs, and so on. We define the belief of order $l$ for agent $i$ as the distribution of other agents' beliefs at order $l-1$ given information available to agent $i$:
\begin{align*}
    B^0_t(i) &\defeq p(S_t|H_t(i)) \, , \\
    B^{l}_t(i) &\defeq p\left(B_t^{l-1}(j)_{j \not = i}|H_t(i)\right) \text{ for } l\geq 1 \, .
\end{align*}
The question of how to represent and compute these belief states is even more prominent than in single-player games, given their recursive nature. As a tractable solution to this problem, we combine the idea of learning higher order beliefs in multi-agent games with that of representing belief states as neural codes. We detail the proposed method in the next section.

\subsection{Neural recursive belief states}\label{sec:rnbs}

We propose learning recursive belief models from agent experience. Following the principle of decentralized training (i.e.\ without a centralized critic) and decentralized execution, we assume that we have access to the environment state and agent histories in hindsight.\footnote{This is a common human learning behaviour. For instance, in a game of cards we could look back into played games and the hands that each player had.} At training time, we provide the agents with a handcrafted state, which captures important information about the full state (this is merely done to aid speed of learning). We re-define $S_t$ to denote the hand-crafted state. During training, we generate \textit{trajectories} from the $n$ players $\tau_t = (S_t, H_t(1), \ldots, H_t(n))$.

\textbf{Learning zeroth-order beliefs}. Agent $i$ learns $B^0_t$ by combining an RNN that computes the neural code $\hat{b}^0_t(i) \defeq f^b_\theta(\hat{b}^0_{t-1}(i), Y_t(i))$), with a parametric generative model that maps the neural belief state $\hat{b}^0_t(i)$ to a distribution $p_\phi(S_t|\hat{b}^0_t(i))$. The generative model can take any form and outputs a distribution in a very large space. The only requirement is efficient computation of its log likelihood $\log p_\phi(S_t|\hat{b}^0_t(i))$. This model can be learned by minimizing the following loss over $\theta$ and $\phi$,
\begin{align}
    \mathcal{L}^0(\theta, \phi) &= - \expec_{p(\tau_t)} \log p_{\phi}(S_t|\hat{b}^0_t(i)) \, ,
\end{align}
where $\hat{b}^0_t(i)$ is the neural belief state as a function of the entire history $H_t(i)$ and of $\theta$, and the gradient is computed using backpropagation through time. 

\noindent \textbf{Learning higher-order beliefs}. In relation to theory of mind, our proposed approach is based on the following questions: (i) \emph{what would I have known if I had observed what the others have observed?}, followed by (ii) \emph{given what I have observed, what do I think the others know?} We first consider the case of two agents, and present the generalization to $n$ agents at the end of this section. For  simplicity, we drop the time-step index below. Consider a pair of agents $i$ and $j$. We must derive learning algorithm for the belief of agent $i$ of order $l$ (about the belief of agent $j$ of order $l-1$). Na\"ively, one might try to model the entirety of the knowledge agent $j$ may have, its entire history $H(j)$. While conceptually desirable, modeling entire histories of observations is computationally difficult. Moreover, it does not truly represent the state of knowledge inferred by agent $j$. Another option is to model the belief of order $l-1$ of agent $j$ directly, by learning a generative model $p(\hat{b}^{l-1}(j)|\hat{b}^l(i))$.  However, it is difficult to define a likelihood on the space of neural codes, as distances in that space are not indicative of the distance between the corresponding distributions. Instead we assume that the generative models corresponding to neural belief states at different orders can readily be sampled. Recall that a distribution can be empirically approximated by a collection of samples. A belief of order $0$ can be approximated by a collection of states $b^{0}(j) \defeq \left(s^{(1)}(j), \ldots, s^{(K)}(j)\right)$. A belief of order $1$ can in turn be approximated by a collection of collections of states. Following the recursion, beliefs of any order are represented by a nested collection, where the innermost constituents are collections of states. Agent $i$'s belief model of order $l$ is approximated by a collection of beliefs of order $l-1$ as $b^{l}(i) \defeq \left(b^{l-1,(1)}(j\ne i), \ldots, b^{l-1,(K)}(j \ne i)\right)$. Representing hierarchical distributions this way is a standard procedure in hierarchical Bayesian learning. When subsets of data are assumed to come from latent components, these are referred to as grouped data \cite{doi:10.1198/016214506000000302, Vandermeulen2015OnTI}. We propose learning hierarchical latent variable models, as these naturally capture the notion of distributions (of distributions, etc.). The latent variables can readily model the i.i.d.\ structure of nested samples that represent a target belief. Specifically, we employ a hierarchy of $l$ latent variables $Z_1, \ldots, Z_l$, defining 
\begin{equation}
    p_\phi(S|\hat{b}^l(i)) \defeq \int_{Z_1,\ldots, Z_l} p_\phi(Z^l | \hat{b}^l(i)) p_\phi(S|Z_1, \hat b^l(i)) \prod_{m=2}^l p_\phi(Z^{m-1}|Z^{m}, \hat b^l(i))
\end{equation}
as a model for the belief of order $l$. In order to generate a nested sample representation from such model, we follow the process illustrated in Fig. \ref{fig:generative_model} (note that the conditioning of the neural code is not shown). We first sample $K$ possible values for the variable $Z_l$, and, conditioned on each of the sampled values $z^{l, (k)}$, we again sample $K$ variables $z^{l-1}$. We recurse this process until all that remains is to sample $K$ state values from $p(S|z^1, \hat{b}^l(i))$.\footnote{Using the same sampling factor $K$ at every level is a particular choice made for simplicity, but one can use different values as needed. } It remains to explain how to learn the neural code of order $l$, which goes back to the two questions posed. An agent learns its belief models by having access to the history of the other agent. That is, the agent infers the neural code of agent $j$ by using its own internal RNNs on $H_t(j)$, and generates the nested sample $b^{l-1}(j)$. This refers to question (i). The learning objective is therefore to model $b^{l-1}(j)$ conditioned on its own neural code $\hat b^l(i)$, addressing question (ii). The learning objective relies on trajectories generated with samples from the belief models $\tau_t = (S_t, \tau_t(1), \ldots, \tau_t(N))$, where $\tau_t(i)=(H_t(i), b^1_t(i), \ldots, b^l_t(i))$. Formally, loss is then given by
\begin{align}
\mathcal{L}^{l}(\theta, \phi) &= - \expec_{p(\tau_t)} \log p_\phi(b^{l-1}(j)|\hat b^{l}(i)) \, .
\label{eq:order_l_loss}
\end{align}
This loss involves a marginalization of the latent variables which is intractable for all but the simplest cases. We can instead use variational inference by maximizing the evidence lower bound (ELBO), and use stochastic variational inference and the re-parameterization trick to obtain efficient gradients over $\phi$. This is known as the variational auto-encoder (VAE) \cite{conf/icml/RezendeMW14, kingmaW13}. The idea of using VAEs to learn distributions of distributions this way is related to the neural statistician \cite{DBLP:conf/iclr/EdwardsS17}. We describe further details regarding the objective function in Appendix \ref{sec:appendix_vae_beliefs}.
%
\begin{figure}[htb]
\subcaptionbox{A second-order generative model and its nested representation for a sampling factor $K=2$.\label{fig:generative_model}}[0.48\textwidth]{
    \includegraphics[width=0.48\textwidth]{figures/hierarchical_model.pdf}
    }
    \hspace{1em}% Space between image A and B
    \subcaptionbox{Agent with belief model. Black arrows are components of recurrent networks, red arrows denote belief models, blue arrows refer to policy and value. \label{fig:architecture} }[0.38\textwidth]{
    \includegraphics[width=0.38\textwidth]{figures/agent_rl_gm_architecture.pdf}
 }
 \caption{Generative model and agent architecture.}
\end{figure}
%
To summarize, $\hat b_t$ is an agent's \emph{neural recursive belief state}, an internal representation of the belief in the form of neural codes $\hat b_t \defeq (\hat b^{0}_t, \dots, \hat b^{l}_t)$. The code at order $l$ conditions the belief distribution $B_t^{l}$ over another agent's corresponding nested samples $b_t^{l-1}$. In the $n$-player case, it is the same method but involves an expansion of $n-1$ beliefs (in relation to each of the other agents) at every level of the recursion. Further discussion is in Appendix \ref{sec:appendix_n_players}. Note how the computational complexity scales exponentially as $\mathcal{O}\left((nK)^l\right)$. Fortunately, we can control the sampling factor according to computational availability, and in practice we expect strong diminishing returns from higher order reasoning. 

There are a number of benefits of our proposed sample-based approach. First, the belief models are ultimately grounded on a well-defined space (the state). Second, the method allows for an efficient decentralized implementation in which agents only require access to the histories of other agents (instead of requiring access to the  models themselves). Finally, it side-steps the intractability of solutions that rely on explicit belief filtering.

\noindent \textbf{The importance of multiple grouped samples}. A na\"ive version of our approach is to model nested single samples ($K=1$), instead of joint nested collections of samples. This method, however, can fail to capture the true distribution of the target beliefs, potentially limiting the ability of agents to compute optimal policies. To see how this applies to learning a first-order belief, consider the following version of the game of Tiger originally proposed as a toy example for single-agent POMDPs \cite{kaelblingLC98}. A player (P1) is faced with two rooms, one with a tiger and one with a prize.  The state of the game is the binary variable $S_t \in \{TL, TR\}$ (whether the tiger is behind the left or right door). P1 can open one door or wait and listen. When P1 chooses to listen, there is a $50\%$ chance of the tiger growling which reveals its door to P1. Clearly, P1 should listen until the tiger growls, and proceed to open the other door. On each round, a second player (P2) passively listens from further away, and can hear whether the tiger growled or not, but cannot tell from which door the growl came. Intuitively, when the tiger growls, P2 becomes certain that P1 is certain of where the tiger is; if instead P2 does not hear a growl, it knows with certainty that P1 is uncertain of the location of the tiger. Formally, P2 has a first-order model $B_t^1(\text{P2})$ of P1's model $B^0_t(\text{P1}) = p(S_t|H_t(\text{P1}))$. Crucially, if P2 learns $B_t^1(\text{P2})$ from one sample $s^{(1)}_t(\text{P1}) \sim B^0_t(\text{P1})$, it will learn over many episodes that 
\begin{align*}
p(B^0_t(\text{P1})=\text{TL}|Y_t(\text{P2})=\text{growl}) =  p(B^0_t(\text{P1})=\text{TL}|Y_t(\text{P2})=\text{silence}) &= 0.5  \, .
\end{align*}
This is because the marginal probability of the tiger's location is always $50\%$ on either door. Thus, P2 cannot know whether P1 will open a door or listen again if it uses this model. On the other hand, if P2 learns to model a collection of samples ${(s_t^{(1)}(\text{P1}),\dots, s_t^{(K)}(\text{P1}))}$, then P2 will know that 
\begin{align*}
&p\left(B_t^{0,(1)}(\text{P1})=\cdots=B_t^{0,(K)}(\text{P1})=TL|Y_t(\textrm{P2})=\text{growl}\right)=0.5, \text{ and} \\ 
&p\left(B_t^{0,(1)}(\text{P1})=\cdots=B_t^{0,(K)}(\text{P1})=TL|Y_t(\text{P2})=\text{silence}\right)=0.5^K \, ,
\end{align*}
since hearing the growl introduces conditional dependence. Because the probabilities are different depending on whether the tiger growls or not, P2 forms the correct belief of P1's belief. This would allow P2 to predict whether P1 would chose to listen or not. In our experiments, we implement this game as an RL environment and train agents that showcase the need for learning correct beliefs in order to learn optimal policies. In Appendix \ref{sec:appendix_tiger_b2}, we also extend this game to a version with a third player that has to form a second order belief.

\subsection{Agent architectures}
While above we defined a different neural code for every belief order, in practice $\hat b_t$ can be implemented by a single code. The agent architecture used in the experiments is an extension to a standard deep architecture with an RNN: it is composed of two recurrent components which aggregate the history of observations to produce a representation as shown in Fig.\ \ref{fig:architecture}. By separating the internal representation into two, a model-free part and a belief representation part, we decouple interactions between the gradient signals of the RL and belief losses which we empirically saw to be helpful. \footnote{The ``stop gradient'' components ensure this decoupling during the learning phase. Both recurrent states are concatenated to produce the complete agent representation for the policy and value prediction.} The two \textit{observation encoders} are composed each of a convolutional neural network (CNN), connected to a multi-layered perceptron (MLP). The encoded observations are inputs to the RNN, which are implemented as GRUs \cite{ChoMGBBSB14}. The outputs of each RNN serve as inputs to both the belief models as well as the policy and value components. The latter are MLPs that produce the action probabilities and the critic of the current state. Specific details of the networks architecture is detailed in Appendix \ref{sec:appendix_agent_architectures}.

\section{Experiments}\label{sec:experiments}

\subsection{Environments}

Our aim is to evaluate the usefulness of using belief models in MARL agents. To do so we describe two environments below, and provide further details and illustrations in Appendix \ref{sec:appendix_games}.

\textit{Running with Scissors} is a partially observable, pure-conflicting interest task extending the classic matrix game rock-paper-scissors to an intertemporal gridworld environment \cite{vezhnevets2019options}. Two players move around a small environment ($15\times23$) and collect resources. Resources have three types (rock, paper, and scissors), which are visually distinguishable from one another. To maximize the reward, players should correctly identify which resource the opponent is collecting and then collect as many counter-resources as possible. Each episode automatically times out after 1000 steps. The hand-crafted state used to build the belief models is defined to be the (private) collected number of rocks, papers, and scissors.

We formalize the \textit{Tiger game} described above as an RL environment. The first player P1 has to choose one of two doors: one has a prize (reward of 1), and the other one a tiger (-5 reward). At every step, the player has 3 actions, open left door (OL), open right door (OR) or listen (L). Listening gives no reward, and the game ends when a door is opened. The task of P2 is to guess at each round whether P1's action is to open a door or to wait and listen based on its observation (with a reward of 1 with the correct guess, or 0 otherwise).

\subsection{Training setup}
The training regime in Running with Scissors is based on \emph{multiple population play}, where a number of agents are sampled from different sub-populations to play in each game. Each sub-population consists of a number of agents of a similar type, each of which has an independent set of network parameters. For each episode, the required number of agents for the game are randomly chosen from the pool of all agents. We distinguish three sub-populations. The \textit{specialist agents} (S), which are trained with a combination of the task reward and pseudorewards designed to produce interpretable policies. In Running with Scissors, these include an agent with high preference for collecting rocks, one for collecting scissors, and one for paper. These specialist agents receive a pseudoreward of $+5$ for collecting the item of their preference. The second sub-population of agents are \emph{non-specialist} agents (NS), which simply learn to maximize the task rewards. The third sub-population comprises the \textit{main agents} we wish to evaluate. The type will vary in every experiment so we can compare the types under the same training regime. These types include agents that use the $B^0$ belief model (B0 agents), agents with first order belief models (B1 agents), and two types as baselines. First is a sub-population of model-free agents in which the architecture of the agent is the same as the agents with belief models, but both RNNs are used solely to estimate the policy and value (these agents also have belief models, but the gradients from belief models do not update the RNN parameters). This allows us to have a fair comparison of model-free and belief agents in terms of number of parameters (with the model-free baseline having overall more trainable parameters for the policy due to the second RNN). The second baseline involves agents that has a predictive model of the opponents trajectory (Tr.\ agent). These agents learn to predict the actions and visual observations of the other agents at every time-step using the second RNN (details in Appendix \ref{sec:appendix_trajectory_agent}). The difference in performance between B0 and Tr.\ agents can highlight the advantage of predicting the salient hand-crafted states in contrast with predicting the opponents' actions and observations.

The training process for both environments uses the distributed actor-critic setup of the Importance Weighted Actor-Learner Architecture \cite{impala2018} (but other RL algorithms are also compatible). Each actor generates trajectories, which are sent to the learner in chunks of 100 environment steps. The learner then optimizes the RL and belief losses jointly. Further details on hyper-parameters used are given in Appendix \ref{sec:appendix_agent_architectures}.

\noindent \textbf{Running with Scissors}.  We first experiment with a multiple population set-up which has three specialist agents, three non-specialist, and one main agent for the third sub-population.  Fig.\ \ref{fig:rws_7joint} shows the average return obtained by the different types of of the main sub-population. We see how both agents with $B^0$ and $B^1$ beliefs clearly outperform the baselines. Also, predicting the opponent's actions and observations does not provide useful representations for the task as seen by the poor performance of the agent with a trajectory-prediction model. To test the hypothesis that higher order reasoning should outperform lower order, we run an experiment which involves two populations of three B0 agents and three B1 agents. We observe in Fig.\ \ref{fig:rws_b0vb1} how B1 agents achieve higher average return than the lower-order counterpart. We also analyze the correlation between average return obtained by these different types and their average belief losses. As we would expect, better belief predictive models lead to higher rewards. Fig.\ \ref{fig:rws_symmetric_scatterb0} shows the correlation with respect to 0th order belief loss. Fig.\ \ref{fig:rws_symmetric_scatterb1} shows the 1st order belief loss for the B0 vs. B1 agents. These results suggest that both belief models enable the agents to infer useful information from their experience.
%
\begin{figure}[ht]
     \centering
     \begin{subfigure}[t]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rws/rws_7joint.pdf}
         \caption{Main agent performance in experiments with 3 S, 3 NS and 1 main agent, per main agent type (6 independent runs). }
         \label{fig:rws_7joint}
     \end{subfigure}
     \hspace{0.5em}
     \begin{subfigure}[t]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rws/rws_b0vb1.pdf}
         \caption{Average return of experiments with 3 B0 and 3 B1 agent populations (8 independent runs).}
         \label{fig:rws_b0vb1}
     \end{subfigure}
     \hspace{0.5em}
     \begin{subfigure}[t]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rws/rws_symmetric_scatterb0.pdf}
         \caption{$L^0$ loss and average rewards correlations on the experiments with 3 S, 3 NS and 1 main agent, per main agent type.}
         \label{fig:rws_symmetric_scatterb0}
     \end{subfigure}
     \hspace{0.5em}
     \begin{subfigure}[t]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rws/rws_symmetric_scatterb1.pdf}
         \caption{$L^1$ loss and average rewards correlations on the experiments with 3 B0 and 3 B1 agents populations.}
         \label{fig:rws_symmetric_scatterb1}
     \end{subfigure}  
    \caption{Training results in Running with Scissors. Shaded areas represent the 95\% confidence intervals for the means averaged over a number of experiment runs.}
    \label{fig:rws_results}
\end{figure}
%
In summary, we see agents with belief representations outperform the baselines in Running with Scissors by identifying the strategies of their opponent in real time and deploying counter-strategies. 

\noindent \textbf{Tiger game}. The Tiger game proposed above is a toy problem designed to  conceptually highlight the potential issues of incorrect modelling of beliefs. We  therefore empirically evaluate whether our representation learning method enables solving the games by computing the correct beliefs.

\begin{figure*}[!htb]
     \centering
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/tiger_b1.pdf}
         \caption{Average return obtained by P2 agents trained with either a belief model learned from K=10 or K=1 samples (from the B0 model of P1).}
         \label{fig:tiger_b1}
     \end{subfigure}
     \hspace{0.5em}
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/tiger_b2.pdf}
         \caption{Average return obtained by P3 agents trained with either a belief model learned from K=10 or K=1 samples (of the B1 model of P2).}
         \label{fig:tiger_b2}
     \end{subfigure}
        \caption{Tiger experimental results when playing against optimal players and optimal beliefs. The optimal policy is denoted by a black dashed line.}
        \label{fig:tiger_results}
\end{figure*}

We experiment with the two versions of the Tiger game to evaluate the ability to learn agents' beliefs and use these beliefs to learn the policies via RL. We run these experiments following the same training method and architecture as detailed in Appendix \ref{sec:appendix_agent_architectures}. 
In the first experiment, we match P2 with an ``optimal'' P1 in the version of the game with two players. The input to the policy and value functions for P2 is thus composed of samples $b_t^1(P2)$ from its own belief model (thus, if the model is correct, the policy should be able to learn how to map these samples to the right actions).
In the second experiment, we evaluate the second version of Tiger with three players. We match P3 against an optimal P2, and learn the policy and value conditioned on $b_t^2(P3)$. We observe in Fig.\ \ref{fig:tiger_results} how in both cases, only the agents that learn from $K=10$ samples can solve the problem, while agents that learn from $K=1$ samples (i.e.\ theoretically unable to learn the correct higher order beliefs) catastrophically fail.


\noindent \textbf{Effect of the nested sampling factor $K$.} Above we showed that in the Tiger game, it becomes impossible to learn the correct distribution with one grouped sample at a time. While conceptually we know that the larger the sampling factor, the better the distributions are approximated, we also investigate in Running with Scissors the empirical effect of representing the nested beliefs with $K=1$, in contrast to a larger value $K=10$. We run experiments in Running with Scissors, where we compare the performance of an agent's first order reasoning using $K=10$, with one using $K=1$. We observe in Fig.\ \ref{fig:rws_b0vb1_repeat} how the B1 agents achieve higher average returns than the B0 agent. However, Fig.\ \ref{fig:rws_b0vb1_1sample} shows that if B1 models are only learned with one sample at at time, B1 agents fail to outmatch the B0 agents, and in fact seem to be doing slightly worse (with a larger variability in performance across 8 runs).

\begin{figure}[!htb]
     \centering
     \begin{subfigure}[t]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rws/rws_b0vb1_10s.pdf}
         \caption{Average return of experiments with 3 B0 and 3 B1 ($K=10$) agent populations (8 independent runs).}
         \label{fig:rws_b0vb1_repeat}
     \end{subfigure}
     \hspace{0.5em}
     \begin{subfigure}[t]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rws/rws_b0vb1_1sample.pdf}
         \caption{Average return of experiments with 3 B0 and 3 B1 ($K=1$) agent populations (8 independent runs).}
         \label{fig:rws_b0vb1_1sample}
     \end{subfigure} 
        \caption{Training results in Running with Scissors. Shaded areas represent the 95\% confidence intervals for the means averaged over a number of experiment runs.}
        \label{fig:b0_b1_samples}
\end{figure}


\section{Related work}\label{sec:rel-work}

The state-of-the-art in learning and leveraging belief models in multi-agent deep RL is the PR2 agent \cite{DBLP:conf/iclr/WenYLWP19}. This algorithm learns a model of others' policies and incorporates this into its update step based on Bayesian reasoning, which leads to the discovery of optimal equilibria in simple coordination problems like matrix games and particle worlds. However, the method is computationally expensive, and it is not clear how well it would scale to more complex tasks with populations of co-players and competitive dynamics. Similarly the BAD \cite{DBLP:conf/icml/FoersterSHBDWBB19} and SAD \cite{anonymous2020simplified} algorithms learn belief models, but are specialized to fully cooperative games. Theory of mind models were proposed in the context of agents with social influence \cite{DBLP:journals/corr/abs-1810-08647}, leading to emergent communication and cooperation in social dilemmas. Unlike our model, successfully leveraging these beliefs requires an intrinsic motivation. The work of \cite{vezhnevets2019options} proposes a hierarchical agent (OPRE), applied also to Running with Scissors, that discovers options useful for strong generalization. 
Our work does not address generalization but rather focuses on
learning representations that support higher opponent awareness and, as a consequence, better decision making.
Our methods are thus not directly comparable; in fact, the latent options discovered by OPRE could be used alongside the representations learned to capture higher order reasoning. 

In single-agent RL, the two primary research aims of previous work in learning belief models have been representation richness and improved task performance in POMDPs. This applies both to works that investigate unsupervised learning techniques \cite{venkatraman2017predictive,IglZLWW18,buesing2018learning,guo2018neural,gregor2019shaping} or leverage supervision on state information  \cite{moreno2018neural,humplik2019meta}. These works, however, do not address the multi-agent setting. 

The field of epistemic game theory studies the reasoning of agents and their beliefs in a formal manner which has lead to a deeper understanding of these notions and to novel solution concepts, see e.g.\ \cite{RePEc:wsi:igtrxx:v:16:y:2014:i:01:n:s0219198914400015} for a historical account. However, the analyses in this field do not usually provide practical solutions to RL in complex environments. Our work is related to the interactive POMDP (iPOMDP) formalism \cite{gmytrasiewicz2005framework} with respect to the notion of recursive belief states, but the intractable formulation of a iPOMDP limit its application to small-scale problems. While some works propose approximations to improve the applicability of iPOMDPs \cite{doshi2009monte, han2019ipomdp}, these methods still do not address the intractability of having to explicitly compute the belief updates.


\section{Conclusion}
We have investigated the use of deep generative models to learn the recursive belief structures that emerge in POMGs. The proposed approach offers a practical framework for learning belief models that are useful in complex environments as shown in our experiments. In future work, we wish to evaluate in greater detail the empirical effects of the sample-size in learning the belief models, and to understand the effects of incorporating higher-order belief models ($B^2$ and higher), which may be important in scenarios requiring deep theory of mind, such as Hanabi \cite{DBLP:journals/corr/abs-1902-00506}. 
